Distributed Clustering of Linear Bandits in Peer to Peer Networks

We provide two distributed confidence ball algorithms for solving linear bandit problems in peer to peer networks with limited communication capabilities. For the first, we assume that all the peers are solving the same linear bandit problem, and prove that our algorithm achieves the optimal asymptotic regret rate of any centralised algorithm that can instantly communicate information between the peers. For the second, we assume that there are clusters of peers solving the same bandit problem within each cluster, and we prove that our algorithm discovers these clusters, while achieving the optimal asymptotic regret rate within each one. Through experiments on several real-world datasets, we demonstrate the performance of proposed algorithms compared to the state-of-the-art.

==> NewMaterial.tex <==
We prove a cummulative regret bound for CB-\emph{delayed} for a general
\begin{theorem}\label{thm:Main-delayed}
With probability $1-\delta$, the regret of CB-\emph{delayed}, where the information used by each agent at each round, $t$, contains at least all the information up to round $\tau(t)$, is bounded by
\begin{align*}
\cR_t
	\le e^{\frac{1}{2}}\left(\beta(t) + R\sqrt{2} \right)
		  	  \sqrt{ |V|t \ln\left(\frac{\det(A_t)}{\det(A_0)}\right) }
		  + \nu(t) \|\theta\|_2
					,
\end{align*}
where
\begin{align}
\label{eq:def-of-beta-delayed}%
\beta(t)
  := R\sqrt{2\log \left(\frac{\det\left(A_t \right)^{1/2}}
  											{\delta\det(A_0)^{1/2}}
  									\right)}
  	  + \frac{\|A_0\|_2\| \theta\|_2}{\lambda_{\min}(A_0)}.
\end{align}
and
\begin{align}
\nu(t) := \Delta(t)^{3} \left(d+\frac{1}{\Delta(t)}\right)d\left(tr\left(A_0^{-1}\right)
			 					-\frac{1}{\Delta(t)}\right),
\ 
\Delta(t) := |V|\max_{1\le k\le t}(k - \tau(k)). \label{eq:nu-delayed}
\end{align}
\end{theorem}
\begin{remark}
Notice that the impact of the delay in the regret bound is additive, and described by $\nu(t)$. Thus if $\nu(t)$ helps to define a trade-off between communication cost of the protocol, and the extra regret incurred by the algorithm.
\end{remark}
Choosing $A_0 = I$ and using that the action spaces $\cD_t^i$ are bounded, we can simplify this bound on the regret as in \cite{abbasi2011improved}.
\begin{corollary}\label{cor:CB-delayed}
Assume $A_0 = I$.
With probability $1-\delta$, the regret of DCB is bounded by
\begin{align*}
\cR_t
	\le& e^{\frac{1}{2}}R\left(  \sqrt{\ln \left({\left(1 + \frac{|V|t}{d} \right)^d}{\delta}\right)}
		 						 + \| \theta\|_2 + \sqrt{2}
		 						 \right)
 		\sqrt{|V|t \ln\left( \left(1+|V|t/d\right)^d\right) } \\
		 & + (|V|\max_{1\le k\le n}(k - T(k)))^3(d+1)d^2\|\theta\|_2.
\end{align*}
\end{corollary}
\begin{remark}
\label{remark: comparison-delayed}
Note that using the results in \cite{abbasi2011improved}, the equivalent regret bound for $|V|$ agents individually solving the same linear bandit problem by implementing CB with no information sharing would be
\begin{align}\label{eq:regret_CB-delayed}
\cR_t
	\le |V| R\left(  \sqrt{\ln \left(\left(1 + t/d \right)^d/\delta\right)}
							+ \| \theta\|_2
							\right)
		\sqrt{t \ln\left( (1+t/d)^d\right) }
\end{align}
Comparing Corollary \ref{cor:CB-delayed} with \eqref{eq:regret_CB-delayed} tells us that, if information sharing happens sufficiently regularly, CB-\emph{delayed} has better cummulative regret performance than CB-\emph{NoSharing} by a factor of almost $\sqrt{|V|}$.
\end{remark}

\subsubsection*{Communication Complexity}
First, suppose that the agents want to communicate their information to each other at each round without a central server, and implement CCB in this way. Then every agent would need to communicate their chosen action and reward to every other agent at each round. Thus the per-round communication cost would be $O(d|V|^2)$.

Suppose that each the total number of rounds before time $t$ at which communication has occured is given by $s(t)$.
Then up to time $t$ a total of $O(s(t)d^2|V|^2)$ bits are be communicated across the network.

\subsubsection*{Proof of Theorem \ref{thm:Main-delayed}}
In this analysis we need to show that the bias introduced by the delayed feedback has a negligible impact on the estimation of the parameter $\theta$.
The proof builds heavily on the analysis in \cite{abbasi2011improved}. 
We give our analysis for a general delay function $\tau = \tau(t)$. 

\paragraph{Step 1: Define modified confidence ellipsoids. }
First we recall the confidence ellipsoid theorem given in \cite{abbasi2011improved}, written to incorporate the delayed feedback:
\begin{proposition}\label{prop:concentration-delayed}
Let $\delta>0$, and let
\begin{align}\label{eq:ellipsoid_1-delayed}
C_t
	:= \left\{ x \in \bR^d : \| \theta_{\tau(t)} - x \|_{A_{\tau(t)}} 
											\le R \sqrt{2\log\left(\frac{\det(A_{\tau(t)})^{\frac{1}{2}}}
																							   {\det(A_0)^{\frac{1}{2}}\delta}\right)}
															+ \frac{\|A_0\|_2\| \theta\|_2}{\lambda_{\min}(A_0)}
					\right\},
\end{align}
where $\theta_t:=A_t^{-1}b_t$.
Then with probability $1-\delta$, $\theta\in C_t$.
\end{proposition}
In the rest of the proof we assume that the event $\theta\in C_t$ holds.

\paragraph{Step 2: Instantaneous regret decomposition.} Let $(x_t^i,\theta_t^i) = \argmax_{x\in D_t^i, y \in C_t} x\tr y$ and $\theta_t := A_{\tau(t)}^{-1}b_{\tau(t)}$. Then we can give a simple decomposition of the instantaneous regret, following the classic argument (see the proof of Theorem 3 in \cite{abbasi2011improved}):
\begin{align*}
\rho_t^i =  \left(x_t^{i,\ast}\right)\tr \theta -  (x_t^i) \tr \theta 
 &\le \left(x_t^i\right)\tr \theta_t^i -  (x_t^i) \tr \theta
  = \left(x_t^i\right)\tr\left[ \left( \theta_t^i -  \theta_t\right) 
		+ \left( \theta_t -  \theta \right) \right]\\
  &\le \| x_t^i \|_{A_{\tau(t)}^{-1}}
  		\left[ \left\| \theta_t^i -  \theta_t\right \|_{A_{\tau(t)}}
		+ \left\| \theta_t -  \theta \right\|_{A_{\tau(t)}} \right]
\end{align*}

\paragraph{Step 3: Control the bias coming from the delay.}

We need to understand the effect of using $A_{\tau(t)}$ in place of $A_t$ in the simple regret decomposition just derived. To this end, let $(y_k)_{k\ge1}$ be any sequence of vectors such that $\|y_k\|_2^2\le 1$, and let $B_n := B_0 + \sum_{k = 1}^{n} y_k y_k\tr$, where $B_0$ is some positive definite matrix. Let $T(\cdot)$ be an arbitrary, monotonically increasing function such that $1\le \tau(t)\le t$ for all $t\ge 1$. Then the following lemma holds:
\begin{lemma}[Bound on the influence of general weights]\label{lem:cov-matrix-det-delayed}
For all $t>0$,
\begin{enumerate}[(i)]
	\item $\det \left(B_{\tau(t)} \right)
					\le \exp \left( \sum_{k = \tau(t)+1}^{t} \| y_k \|_{B_k^{-1}}^2\right)
																		\det\left(B_t \right)$,
	\item \label{lem:cov-matrix-det-delayed-ii} and $\| y_t \|_{B_{\tau(t)}^{-1}}^2
						\le \exp \left( \sum_{k = \tau(t)+1}^{t} \| y_k \|_{B_k^{-1}}^2\right)
																									\| y_t \|_{B_t^{-1}}^2$.
\end{enumerate}
\end{lemma}

In order to control the size of the exponential factors in the above lemma, we require a further lemma:
\begin{lemma}\label{lem:norm-transf-2-modified}
For all $t>0$, and for any $c\in (0,1)$, we have
\begin{align}
\label{eq:no-of-outliers-delayed}
 \left| \left\{ k \in \{1,2,\dots\}: \|y_k\|_{B_{k-1}^{-1}}^2 > c \right\}\right| 
 	\leq  \frac{(d+c)d(tr(B_0^{-1})-c)}{c^2},
\end{align}
\end{lemma}
Combining these two lemmas we can control the number of times $k\in\{1,\dots,t\}$ at which using $B_{\tau(k)}$ in place of $B_k$ incurs more than a multiplicative constant:
\begin{proposition}[Controlling the bias due to delayed feedback]\label{prop:num-outliers-delayed}
For any $c\in (0,1)$,
\begin{align}\label{eq:B_bound_3_delayed}
&\left|\left\{ k \in \{1,\dots,t\}: \|y_{k}\|^2_{ B_{\Delta(k)}^{-1}}
													\ge c \|y_{k}\|^2_{ B_{k}^{-1}} \text{, or }
												\det \left(B_{\Delta(t)} \right)
													\ge c \det \left(B_{t} \right)\right\}\right|\nonumber\\
	 &\qquad
	 \le \frac{\Delta(t)^{3}}{\left(\ln(c)\right)^2}
	 		\left(d+\frac{\ln(c)}{\Delta(t)}\right)d\left(tr\left(B_0^{-1}\right)
	 					-\frac{\ln(c)}{\Delta(t)}\right),
\end{align}
where $\Delta(t) := \max_{1\le k\le t}\{k - \tau(k)\}$.
\end{proposition}

\paragraph{Step 4: Sum the simple regret.}
Now we are ready to use Proposition \ref{prop:concentration-delayed} in the regret decomposition and apply the lemmas above to mitigate the impact of the delay function $\tau(t)$: setting $(y_k)_{k=1}^{|V|t} = \circ_{k=1}^t((x_k^i)_{i=1}^{|V|})$ in the results from Step 3, we have that
\begin{align}
\rho_k^i
	\le &e^{\frac{1}{2}} \| x_t^i \|_{\left(A_{k-1} + \sum_{j=1}^{i-1}x_{k}^{j} \left(x_{k}^{j}\right)\tr \right)^{-1}}
  					 \left[R\sqrt{2\log \left( \frac{e\det\left(A_{t-1}
  					 													+ \sum_{j=1}^{i-1}x_{k}^{j} \left(x_{k}^{j}\right)\tr \right)^{\frac{1}{2}}}
  					 												{\det\left(A_0 \right)^{\frac{1}{2}}\delta}\right)}
  					 		+ \frac{\|A_0\|_2\| \theta\|_2}{\lambda_{\min}(A_0)}
  					 \right]. \label{eq:simple-regret-delayed}
\end{align}
for at most
\begin{align*}
\nu(t) = \Delta(t)^{3} \left(d+\frac{1}{\Delta(t)}\right)d\left(tr\left(A_0^{-1}\right)
			 					-\frac{1}{\Delta(t)}\right)
\end{align*}
many $k\in\{1,\dots,t\}$, where $\Delta(t) = |V|\max_{1\le k\le t}\{k - \tau(k)\}$.
Now we can conclude that, with probability $1 - \delta$,
\begin{align*}
\cR_t &\le \sqrt{|V|t\sum_{t' = N_\delta}^t\sum_{i = 1}^{|V|}\left(\rho_{t'}^i\right)^2}\\
		&\le \nu(t)\|\theta\|_2
						+  e^{\frac{1}{2}} \left(\beta(t) + R\sqrt{2} \right)\sqrt{|V|t\sum_{t' = 1}^t\sum_{i = 1}^{|V|}  \| x_t^i \|_{\left(A_{k-1} + \sum_{j=1}^{i-1}x_{k}^{j} \left(x_{k}^{j}\right)\tr \right)^{-1}}^2} \\
 		&\le \nu(t) \|\theta\|_2
 						+ e^{\frac{1}{2}} \left(\beta(t) + R\sqrt{2} \right)\sqrt{|V|t \left(2\log\left( \frac{\det\left(A_t \right)}{\det(A_0)}\right)\right) },
\end{align*}
where $\beta(\cdot)$ is as defined as in \eqref{eq:def-of-beta-delayed}.
For the first inequality we have applied Cauchy-Schwarz; for the second inequality we have applied \eqref{eq:simple-regret-delayed} and \eqref{eq:nu-delayed}; for the last inequality we have used Lemma 11 from \cite{abbasi2011improved}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Intermediary Results}
Let $(y_k)_{k\ge1}$ be any sequence of vectors such that $\|y_k\|_2^2\le 1$, and let $B_n := B_0 + \sum_{k = 1}^{n} y_k y_k\tr$, where $B_0$ is some positive definite matrix. Let $\tau(\cdot)$ be an arbitrary, monotonically increasing function such that $1\le \tau(t)\le t$ for all $t\ge 1$. 

\begin{proof}[Proof of Lemma \ref{lem:cov-matrix-det-delayed}]
Let $1<t'\le t$. Then,
\begin{enumerate}[(i)]
	\item we have
\begin{align*}
\det \left(B_t \right)
	=& \det \left(B_t - y_t y_t\tr + y_t y_t\tr  \right)
	= \det \left(B_{t-1} + y_t y_t\tr  \right)
	=\det \left(B_{t-1} \right)
	  				\left(1 + \|y_t\|_{B_{t-1}^{-1}}^2 \right)\\
	=& \det \left(B_{T(t)} + y_t y_t\tr \right)
	  				\prod_{k = T(t)+1}^t\left(1 + \|y_k\|_{B_{k-1}^{-1}}^2 \right)\\
	\le& \exp \left( \sum_{k = T(t)+1}^t\|y_k\|_{B_{k-1}^{-1}}^2\right)
					\det \left(B_{T(t)} + y_t y_t\tr \right)
\end{align*}
The second equality follows using the identity $\det(I+ B^{1/2}x x\tr B^{1/2}) = (1+\|x\|_{B}^2)$, for any matrix $B$ and vector $x$. The inequality follows by taking the exponential of the logarithm, and using that $\ln(1+x)\le x$.
	\item Using the Sherman-Morrison Lemma, and Cauchy-Schwarz inequality we have that, for any vector $x$:
\begin{align}
x\tr (B_t )^{-1}x
	&= x\tr (B_{t-1} + y_t y_t\tr )^{-1}x
	= x\tr B_{t-1}^{-1}x - \frac{x\tr B_t^{-1}y_t y_t\tr B_{t-1}^{-1}x}{1+y_t\tr B_{t-1}^{-1}y_t}\nonumber\\
	&\ge x\tr B_{t-1}^{-1}x - \frac{x\tr B_{t-1}^{-1}xy_t\tr B_{t-1}^{-1}y_t}{1+y_t\tr B_{t-1}^{-1}y_t}
	= x\tr B_{t-1}^{-1}x(1+y_t\tr B_{t-1}^{-1}y_t)^{-1}\nonumber\\
	&\ge \prod_{k = T(t)+1}^t \left(1+\|y_k\|_{B_{k-1}^{-1}}^2\right)^{-1} x\tr B_{T(t)}^{-1}x
	\ge \exp\left( -\sum_{k = T(t)+1}^t \|y_k\|_{B_{k-1}^{-1}}^2\right) x\tr B_{T(t)}^{-1}x\label{eq:sher-morr-trick-delayed}
\end{align}
Taking $x = y_t$ finishes the proof.
\end{enumerate}
\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:norm-transf-2-modified}]
We begin by showing that, for any $c\in(0,1)$
\begin{align}\label{eq:assump-delayed}
\|y_k\|_{B_{k-1}^{-1}}^2 >  c
\end{align}
can be true for only $2dc^{-3}$ different $k$.

Indeed, let us suppose that \eqref{eq:assump-delayed} is true for some $k$. Let $(e_i^{(k-1)})_{1\le i \le d}$ be the orthonormal eigenbasis for $B_{k-1}$, and, therefore, also for $B_{k-1}^{-1}$, and write $y_k = \sum_{i = 1}^d\alpha_i e_i$. Let, also, $(\lambda_i^{(k-1)})$ be the eigenvalues for $B_{k-1}$. Then,
\begin{gather*}
 c
 	< y_k\tr B_{k-1}^{-1} y_k
 	= \sum_{i = 1}^d \frac{\alpha_i^2}{\lambda_i^{(k-1)}}
    \leq \|y_k\|_2^2 \sum_{i = 1}^d \frac{1}{\lambda_i^{(k-1)}}
    \leq \sum_{i = 1}^d \frac{1}{\lambda_i^{(k-1)}}
    = tr(B_{k-1}^{-1} )
,\\
 \implies\ 
  \exists j\in\{1,\dots,d\}:\frac{\alpha_j^2}{\lambda_j^{(k-1)}},\ \frac{1}{\lambda_j^{(k-1)}} >  \frac{c}{d},
\end{gather*}
where we have used that $\alpha_i^2<1$ for all $i$, since $\|y_k\|_2<1$. Now,
\begin{align*}
tr(B_{k-1}^{-1}) - tr(B_k^{-1})
 &= tr(B_{k-1}^{-1}) - tr((B_{k-1}+y_k y_k\tr)^{-1})\\
 &>  tr(B_{k-1}^{-1})  - tr((B_{k-1}+\alpha_j^2e_j e_j\tr)^{-1})
 = \frac{1}{\lambda_j^{(k-1)}} - \frac{1}{\lambda_j^{(k-1)} + \alpha_j^2}\\
 &= \frac{\alpha_j^2}{\lambda_j^{(k-1)}(\lambda_j^{(k-1)} + \alpha_j^2)}
 > \left(\frac{d^2}{c^2} + \frac{d}{c}\right)^{-1}
 > \frac{c}{d}\left(1 + \frac{d}{c}\right)^{-1}
 > \frac{c^2}{d(d+c)}
\end{align*}
So we have shown that
\begin{align*}
\text{\eqref{eq:assump-delayed}}
	\ \implies\ tr(B_{k-1}^{-1} )>  c,
	\text{ and } tr(B_{k-1}^{-1}) - tr(B_k^{-1}) > \frac{c^2}{d(d+c)}.
\end{align*}
Since $tr(B_0^{-1})\ge tr(B_{k-1}^{-1}) \ge tr(B_k^{-1})\ge 0$ for all $k$, it follows that \eqref{eq:assump-delayed} can be true for at most $(d+c)d(tr(B_0^{-1})-c)c^{-2}$ different $k$, which proves \eqref{eq:no-of-outliers-delayed}.
\end{proof}
\begin{proof}[Proof of Proposition \ref{prop:num-outliers-delayed}]
Now, note that, by Lemma~\ref{lem:cov-matrix-det-delayed}, for all $k<t$
\begin{align*}
\|y_{k+1}\|_{B_{\tau(k)}^{-1}}
	\le e^{\sum_{s = \tau(k)+1}^{k}\|y_{s+1}\|_{B_{s}^{-1}}}
																		\|y_{k+1}\|_{B_{k}^{-1}},
\text{ and }
\det \left(B_{\tau(t)} \right)
	\le e^{ \sum_{k = \tau(t)+1}^{t} \| y_k \|_{B_k^{-1}}^2}
																		\det\left(B_t \right).
\end{align*}
Therefore,
$$
\left( \|y_{k+1}\|_{B_{\tau(k)}^{-1}} \geq c \|y_{k+1}\|_{B_k^{-1}}
\text{ or }
\det(B_{\tau(k)}) \geq c \det(B_k)\right)
\implies
\left( \sum_{s=\tau(k)}^{k-1} \|y_{s+1}\|_{B_s^{-1}} \geq \ln(c) \right)
$$
However, according to (\ref{eq:no-of-outliers-delayed}), there can be at most 
\begin{align*}
\nu(t)	:= \frac{\left(d+\frac{\ln(c)}{\Delta(t)}\right)d\left(tr\left(B_0^{-1}\right)-\frac{\ln(c)}{\Delta(t)}\right)}
			{\left(\frac{\ln(c)}{\Delta(t)}\right)^2}
\end{align*}
times $s\in \{1,\dots,t\}$, such that $\|y_{s+1}\|_{B_{s}^{-1}}\ge \ln(c)/\Delta(t)$, where $\Delta(t) := \max_{1\le k\le t}\{k - \tau(k)\}$.
Hence
$\sum_{s=\tau(j)+1}^{k}\|y_{s+1}\|_{B_s}^{-1} \geq \ln(c)$
is true for at most $\Delta(t)\nu(t)$ indices $k\in\{1,\dots,t\}$, which proves \eqref{eq:B_bound_3_delayed}.
\end{proof}
